Inferring Implicit Goals Across Differing Task Models

One of the significant challenges to generating value-aligned behavior is to not only account for the specified user objectives but also any implicit or unspecified user requirements. The existence of such implicit requirements could be particularly common in settings where the user's understanding of the task model may differ from the agent's estimate of the model. Under this scenario, the user may incorrectly expect some agent behavior to be inevitable or guaranteed. This paper addresses such expectation mismatch in the presence of differing models by capturing the possibility of unspecified user subgoal in the context of a task captured as a Markov Decision Process (MDP) and querying for it as required. Our method identifies bottleneck states and uses them as candidates for potential implicit subgoals. We then introduce a querying strategy that will generate the minimal number of queries required to identify a policy guaranteed to achieve the underlying goal. Our empirical evaluations demonstrate the effectiveness of our approach in inferring and achieving unstated goals across various tasks.

==> Cache-built-on-Jan11/0-intro.tex <==
\section{Introduction}


% Why is it interesting?
Humans often omit details they consider obvious, unavoidable, or not worth mentioning when providing instructions. This omission leads to implicit goals and unstated preferences that AI systems must navigate to truly align with human intentions. In various tasks, certain steps or conditions might be critical given the chosen approach and environmental constraints. We refer to these critical points as \textit{bottleneck states}, some of which may represent implicit goals essential for alignment.
Bottleneck states are key waypoints or conditions that must be met to progress toward the goal in a manner consistent with human expectations. They represent crucial decision points that, if bypassed, could lead to solutions that are technically correct but misaligned with the user's true intentions.

% People often omit details they consider obvious, unavoidable, or simply not worth mentioning. This leads to \textit{implicit goals} and unstated preferences that AI systems must navigate. In a navigation task, for instance, crossing a particular bridge or passing by a specific landmark might be necessary given the chosen mode of transportation and the city's layout. These critical points that must be traversed are what we call \textit{bottleneck states}. Some of these bottleneck states may be implicit goals.
% Bottleneck states are essential waypoints or conditions that must be met to progress toward the goal, given a particular approach or set of constraints. They represent key transitions or decision points in the journey that cannot be bypassed without significantly altering the nature of the task or the method of completion.

Consider an agent tasked with guiding a tourist to a famous art museum. The tourist simply says, ``Get me \textcolor{red}{a plan to get} to the art museum," unaware of the city's metro system and expecting an above-ground route passing certain landmarks. The agent, however, might plan a route using the metro system.
In this scenario, bottleneck states are unavoidable points that must be traversed to reach the goal, given certain constraints. For the agent's metro route, these include entering the metro, making transfers, and exiting at the correct station. For the tourist's expected route, they might include crossing a river and passing through the city center.
This misalignment stems from differing world models: the agent's comprehensive transit data versus the tourist's limited knowledge of the city's layout. The challenge in AI alignment lies in bridging this gap – identifying and accounting for implicit aspects of the task that weren't mentioned, and understanding how these relate to unavoidable states in achieving the goal.

% Take the example of an AI assistant tasked with guiding someone to the Louvre in Paris. The human might simply say, ``Get me to the Louvre Museum." This instruction seems straightforward, but it's laden with unspoken expectations. The human has a map of the city but is not aware of metro lines. They expect to pass near the Seine and in front of Notre Dame. They didn't explicitly state these are the intermediate steps they envision, assuming they were self-evident or unavoidable aspects of the trip.
% The AI, however, might plan a route using the metro system. This plan would include necessary steps like entering a metro station, arriving at the correct stop, and exiting the system. While these steps are crucial to reaching the Louvre via metro, they may not align with the human's unstated expectations for an above-ground journey.
% This misalignment stems from differing world models and incomplete specifications. The AI operates on comprehensive transit data, while the human's model is based on different knowledge of the city's layout. The challenge lies in bridging this gap – identifying and accounting for implicit aspects of the task that weren't mentioned, simply because they weren't thought to need mentioning.
% What is the problem you chose to investigate?

% The lack of effective communication of goals between agents with different world models is a significant challenge in artificial intelligence. 
This paper explores how an agent can learn and achieve the implicit goals of another agent, particularly when their understandings of the environment differ.
% Why is it hard?
This problem is particularly challenging due to three main factors: (1) the implicit nature of subgoals, (2) the differences between agents' world models, and (3) the need for efficient information gathering to overcome knowledge gaps. 

% What is a baseline approach to its solution / how has it been solved in the past
Traditional approaches of goal-conditioned reinforcement learning and planning often rely on explicit goal specification or assume shared world models between agents. This can lead to suboptimal or even incorrect task execution in complex, real-world scenarios. % What is your suggested approach ?
We propose a novel approach that leverages the concept of implicit goals within a Markov Decision Process (MDP) framework. Our method aims to compute policies that align with implicit goals by utilizing incomplete knowledge about another agent's model of the world. We formalize the problem using two distinct MDPs: the executing agent's model, the robot, and the goal-setting agent's model, the human. By introducing the notion of bottleneck states and implicit goal sets, we aim to address the discrepancies between these models.

% What are the formal guarantees you provide \/ How do you plan to evaluate the approach ?
To evaluate our approach, we propose empirical evaluations in simulated scenarios. These evaluations will assess the ability to infer and align to implicit goals across various tasks.
% What are the limitations of the suggested approach and how can it be extended ?
Our key contributions include:
\begin{itemize}
    \item Formulation of implicit goals within an MDP framework
    \item Analysis of goal misalignment in the context of MDPs
    \item Introduction of methods to reason about and infer unstated goals across differing world models
    \item Development of novel querying algorithms for efficient information gathering to refine goal understanding
    \item Creation of a framework to learn and satisfy implicit goals using MDPs and information-theoretic querying
    \item Proposal of empirical evaluations in simulated scenarios to assess the ability to infer and align implicit goals across various tasks
\end{itemize}


%By developing this framework to achieve implicit goals using MDPs and information-theoretic querying, we aim to bridge the gap between high-level instructions and nuanced execution in AI systems. This approach allows for the analysis of goal misalignment while providing methods to reason about and infer unstated goals across differing world models.







% We formalize the concept of implicit goals within an MDP framework, allowing for the analysis of goal misalignment. We introduce methods to reason about and infer unstated goals across differing world models, while proposing novel querying algorithms that efficiently gather information to refine goal understanding. By developing a framework to learn and satisfy implicit goals using MDPs and information-theoretic querying, we aim to bridge the gap between high-level instructions and nuanced execution in AI systems. 


% While our approach offers a promising direction for addressing implicit subgoal learning, it has limitations. The current formulation assumes a finite state and action space, which may not fully capture the complexity of all real-world scenarios.

==> Cache-built-on-Jan11/3-form.tex <==
\section{Planning for Implicit Subgoals}
As mentioned before, we are interested in a scenario where the robot's model of the task  $\mathcal{M}^R = \langle S, A, T^R, s_0, \gamma, S_G\rangle$ is different from the user's beliefs about the task $\mathcal{M}^H = \langle S, A, T^H, s_0, \gamma, S_G \rangle$ in terms of the underlying transition function\footnote{Even though we use the term robot to refer to the AI system, nothing in our framework requires the AI system to be physically embodied. Similarly, the user, in theory, could be any principal-agent setting the objective and not necessarily a human user.}. This difference leads the user to overlook specifying subgoals they are confident are bound to happen. 
We will leverage the notion of a {\em bottleneck state}, where a state is said to be a bottleneck state if it is reached in every path from the initial state to the goal. More formally,
\begin{defn}
\label{def:bottle}
 For a given MDP model $\mathcal{M} = \langle S, A, T, s_0, \gamma, S_G \rangle$, we define a \textbf{bottleneck state} as a state $s \in S$ that must be visited by any valid trace starting from $s_0$, for any policy, with non-zero probability of reaching a state in $S_G$. We denote the set of all bottlenecks as $B \subseteq S$. 
\end{defn}

Now, we assume that implicit subgoals ($\mathcal{I}_{G}$) are a subset of $B$ that the user wants the robot to achieve on its way to the goal. From the user's point of view, there is no need to spell out these implicit subgoals since they are bottleneck states in their own model and thus cannot be avoided. However, as the robot and user models differ, what is a bottleneck state in one model may not be in the other. What are interested in here is finding a policy that achieves the subgoals in the robot's models. Formally,
 
% However, this becomes tricky when the model that is executing the policy may not be the 
% A given policy is said to achieve a set of implicit subgoals in the robot model if every trace to the goal in the policy passes through every subgoal. Or more formally,
\begin{defn}
   For a given robot model $\mathcal{M}^R = \langle S, A, T^R, s_0, \gamma, S_G\rangle$, a policy $\pi$ is said to \textbf{achieve a set of implicit subgoal(s)}  $\mathcal{I}_{G}$, i.e., $\pi\models_{\mathcal{M}^R} \mathcal{I}_{G}$, if every goal reaching trace from $s_0$ $\tau \sim_{\mathcal{M}^R} \pi(s_0)$ passes through every state $s \in \mathcal{I}_{G}$. 
\end{defn}
The main challenge we face is to find a policy that achieves all the implicit subgoals when we do not know the implicit subgoals or the exact user model.
% two accommodations
To achieve this, we make the following two reasonable assumptions: (1) We are given a set of potential user models $\mathbb{M}^{H}$ corresponding to different transition functions; and (2) We can query the user about potential implicit subgoals.
We will represent the latter using an oracle function of the form $\mathcal{O}_{\mathcal{I}_G}: S \rightarrow \{0,1\}$, where it can tell you whether a state $s$ is an implicit subgoal or not, i.e.,
\[\mathcal{O}_{\mathcal{I}_G}(s) = 
\begin{cases}
    1~\textrm{if}~s\in \mathcal{I}_G\\
    0~\textrm{otherwise}
\end{cases}
\]
Now, it is worth looking at how reasonable these assumptions are. It is always possible to have access to $\mathbb{M}^{H}$ by taking into account all possible well-formed transition functions that could be formulated for $S$ and $A$. This might result in an infinite set, but one can still formulate it. Similarly, for most cases of interest, such as when a human user is specifying a goal, they would also be able to identify whether or not a state is something they want to achieve.
Note that we are not claiming that the user can formulate an explicit set of all implicit subgoals upfront, but rather they can recognize states they want to achieve. While the former has been shown to fail \cite{Mechergui_Sreedharan_2024}, the latter is the backbone of all methods for learning from user preferences \cite{mechergui2024expectation}.\srm{Change one of this into a different citation.. both being my citation is just asking for trouble}
To make this assumption even more realistic, we will set the cost of querying the user extremely high. The problem then becomes to find the minimal set of queries we need to use to find a policy that achieves the true implicit subgoals.
% problem definition
\srm{extremely handwavy definition}
\begin{defn}
    For a given robot model $\mathcal{M}^R$, a set of possible user models $\mathbb{M}^{H}$, and an oracle $\mathcal{O}_{\mathcal{I}_G}$ for an unknown implicit subgoal set $\mathcal{I}_G$, the problem of \textbf{query identification for implicit subgoals} is to choose states to pass to the oracle, so that the robot can identify a policy $\pi$ that is guaranteed to achieve the implicit subgoal $\mathcal{I}_G$, or that it can never come up with such a policy. 
\end{defn}

Importantly, we are not interested in finding any series of queries but an optimal one. After all, asking about all states $S$ will trivially satisfy this requirement. However, the optimality here depends on the potential subgoals at any instance and the uncertainty of the oracle response. We will see a complete definition of optimal queries later in the paper, but for now, we will rely on a simple recursive definition that builds on the notion of tail subproblem optimality from dynamic programming \cite{Bertsekas2010DynamicPA}.
\begin{defn}
\label{def:optimal}
    At a given instance where the existence of the policy cannot be determined, with a potential set of known implicit subgoals $\mathcal{K}_{\mathcal{I}}$, and not implicit subgoals $\mathcal{K}_{\neg\mathcal{I}}$, a state query $s_q$ is optimal if it meets either of the following condition
    \begin{enumerate}
        \item[c1:](\textbf{Single-step-optimal-solution}) After passing the query to the oracle, the policy's existence can be exactly determined regardless of the outcome. For states that meet this criteria, the cost to go is $1$.
        \item[c2:] (\textbf{Recursive-Optimality}) No single-step optimal solution exists, and the query minimizes the cost to go averaged across each oracle outcome. The cost to go for each outcome is set as 1 + $C_{avg}$, where $C_{avg}$ is the average of the cost over potential outcomes of future queries.
    \end{enumerate}
\end{defn}
In our final formulation, in addition to the cost of queries, we will also introduce the probability of goal achievement as a secondary optimization criterion. 
\textcolor{red}{It is worth noting that this definition can be mapped into an optimal policy for a specific POMDP. The details of the compilation is provided in the supplementary file.}
This treatment of the goal achievement as a secondary optimization criterion follows from the fact that we treat user queries as the biggest bottleneck and need to be given priority. However, our methods can easily be extended to support cases where we know the exact tradeoff between the two components and thus can be combined into a single objective function (see Section \ref{sec:disc}).
% talk about the fact that secondary optimization criteria is the value



==> plots.tex <==

% \begin{figure*}[t]
%     \centering
%     \begin{subfigure}[b]{0.48\textwidth}
%         \begin{tikzpicture}
%             \begin{axis}[
%                 ybar,
%                 bar width=12pt,
%                 width=\textwidth,
%                 height=0.75\textwidth,
%                 symbolic x coords={Maze,Four Rooms,Puddle,Rocks},
%                 xtick=data,
%                 ylabel={Time (seconds)},
%                 ymin=0,
%                 ymax=8,
%                 legend style={at={(0.5,-0.25)}, anchor=north, legend columns=2},
%                 error bars/y dir=both,
%                 error bars/y explicit,
%                 nodes near coords align={vertical},
%             ]
%                 \addplot[fill=blue!40] coordinates {
%                     (Maze,2.6) +- (0.9,0.9)
%                     (Four Rooms,2.0) +- (0.8,0.8)
%                     (Puddle,3.3) +- (1.6,1.6)
%                     (Rocks,2.5) +- (0.9,0.9)
%                 };
%                 \addplot[fill=green!40] coordinates {
%                     (Maze,3.9) +- (1.8,1.8)
%                     (Four Rooms,3.7) +- (0.7,0.7)
%                     (Puddle,4.8) +- (1.4,1.4)
%                     (Rocks,4.8) +- (1.4,1.4)
%                 };
                
%                 % Add significance annotations with manual positioning
%                 \node[text height=12pt] at (axis cs:Maze,6) {$p{=}0.071$};
%                 \node[text height=12pt] at (axis cs:Four Rooms,6) {$p{<}0.001{^{***}}$};
%                 \node[text height=12pt] at (axis cs:Puddle,6) {$p{=}0.085$};
%                 \node[text height=12pt] at (axis cs:Rocks,6) {$p{=}0.012{^*}$};
                
%                 \legend{\strut Strategic Query,\strut Query-All}
%             \end{axis}
%         \end{tikzpicture}
%         \caption{4{\mkern-2mu}×{\mkern-2mu}4 grid environments}
%         \label{fig:grid4x4}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.48\textwidth}
%         \begin{tikzpicture}
%             \begin{axis}[
%                 ybar,
%                 bar width=12pt,
%                 width=\textwidth,
%                 height=0.75\textwidth,
%                 symbolic x coords={Maze,Four Rooms,Puddle,Rocks},
%                 xtick=data,
%                 ylabel={Time (seconds)},
%                 ymin=0,
%                 ymax=10,
%                 legend style={at={(0.5,-0.25)}, anchor=north, legend columns=2},
%                 error bars/y dir=both,
%                 error bars/y explicit,
%                 nodes near coords align={vertical},
%             ]
%                 \addplot[fill=blue!40] coordinates {
%                     (Maze,3.8) +- (1.5,1.5)
%                     (Four Rooms,3.2) +- (1.0,1.0)
%                     (Puddle,4.3) +- (3.3,3.3)
%                     (Rocks,4.1) +- (2.4,2.4)
%                 };
%                 \addplot[fill=green!40] coordinates {
%                     (Maze,6.8) +- (3.9,3.9)
%                     (Four Rooms,3.7) +- (0.7,0.7)
%                     (Puddle,7.7) +- (2.7,2.7)
%                     (Rocks,6.9) +- (3.1,3.1)
%                 };
                
%                 % Add significance annotations with manual positioning
%                 \node[text height=12pt] at (axis cs:Maze,8) {$p{=}0.067$};
%                 \node[text height=12pt] at (axis cs:Four Rooms,8) {$p{=}0.411$};
%                 \node[text height=12pt] at (axis cs:Puddle,8) {$p{=}0.053$};
%                 \node[text height=12pt] at (axis cs:Rocks,8) {$p{=}0.073$};
                
%                 \legend{\strut Strategic Query,\strut Query-All}
%             \end{axis}
%         \end{tikzpicture}
%         \caption{6{\mkern-2mu}×{\mkern-2mu}6 grid environments}
%         \label{fig:grid6x6}
%     \end{subfigure}
%     \caption{Comparison of Strategic Query vs Query-All approaches across different grid sizes. Error bars show standard deviation. Statistical significance: $^*p{<}0.05$, $^{***}p{<}0.001$}
%     \label{fig:comparison}
% \end{figure*}


% First place table spanning both columns at top


==> proofs.tex <==
\begin{proof}[Proof of Proposition 1]
Let $M = \langle S,A,P,R,\gamma,s_0\rangle$ be an MDP and $s_t \in S \setminus {s_0}$ be a state we are testing for being a bottleneck. We will prove by contraposition that if $s_t$ is a bottleneck state, then there must exist an $r < 0$ such that $V^*_{M'(s_t, r)}(s_0) < 0$.
Assume that for all $r < 0$, $V^*_{M'(s_t, r)}(s_0) \geq 0$.
Let $\pi^*$ be an optimal policy for the original MDP $M$. Consider any trajectory $\tau = (s_0, a_0, s_1, a_1, ..., s_n)$ from $s_0$ to a goal state under $\pi^*$.
If $s_t$ is not in $\tau$, then this trajectory remains unchanged in $M'(s_t, r)$ for any $r$, and its value remains non-negative.
If $s_t$ is in $\tau$, let $k$ be the first index such that $s_k = s_t$. The value of this trajectory in $M'(s_t, r)$ is:
$
V_{\tau} = \sum_{i=0}^{k-1} \gamma^i R(s_i) + \gamma^k r + \sum_{i=k+1}^n \gamma^i R(s_i)
$

As $r \to -\infty$, $V_{\tau} \to -\infty$.
However, there must exist at least one trajectory $\tau'$ that doesn't include $s_t$ (otherwise, $s_t$ would be a bottleneck, contradicting our assumption). The value of $\tau'$ remains non-negative in $M'(s_t, r)$ for all $r$.
Therefore, for any $r$, the optimal policy in $M'(s_t, r)$ can always choose $\tau'$ or a similar trajectory that avoids $s_t$, ensuring that $V^*_{M'(s_t, r)}(s_0) \geq 0$.
This contradicts the definition of a bottleneck state, which must be visited by all trajectories from $s_0$ to the goal with non-zero probability.
Thus, if $s_t$ is a bottleneck state, there must exist an $r < 0$ such that $V^*_{M'(s_t, r)}(s_0) < 0$.
By contraposition, if for all $r < 0$, $V^*_{M'(s_t, r)}(s_0) \geq 0$, then $s_t$ is not a bottleneck state.
\end{proof}
\begin{proof}[Proof of Proposition 2]
We prove this by contradiction. Let $s$ be an implicit goal per human for goal $G$ and its bottlenecks $B$. Assume, for the sake of contradiction, that there exists a policy $\pi'$ such that $\pi' \models_{\delta(M^R_h)} (G, B)$ but $\pi' \not\models_{\delta(M^R_h)} s$.

By the definition of determinization, there exists a new action $a_i'$ in $\delta(M^R_h)$ such that $P'(s_i,a_i',s')=1$, for every non-zero transition $P(s_i,a_i,s')$ in $M^R_h$. This means that any trajectory possible in $\delta(M^R_h)$ is also possible in $M^R_h$, just with probability $1$ for each transition.

Given this relationship between $M^R_h$ and $\delta(M^R_h)$, we can construct a corresponding policy $\pi$ for $M^R_h$ from the policy $\pi'$ in $\delta(M^R_h)$ as follows: for each action $a_i'$ in $\delta(M^R_h)$, choose the corresponding action $a_i$ in $M^R_h$ such that if $\pi'(s_i) = a_i'$, then $\pi(s_i) = a_i$.

Due to this construction, if $\pi' \models_{\delta(M^R_h)} (G, B)$, then $\pi \models_{M^R_h} (G, B)$. This is because, by our definition, if there exists any $\tau' \sim \pi'$ that ends in $G$ and passes through all bottleneck states in $B$ in $\delta(M^R_h)$, there must exist a corresponding $\tau \sim \pi$ that ends in $G$ and passes through all bottleneck states in $B$ in $M^R_h$.

Since $s$ is an implicit goal, for all policies $\pi$ such that $\pi \models_{M^R_h} (G, B)$, it must also be true that any trajectory $\tau \sim \pi$ includes $s$. This means that any trajectory $\tau \sim \pi$ that reaches $G$ and passes through all bottleneck states in $B$ must also include $s$.

Given the relationship between $M^R_h$ and $\delta(M^R_h)$, this implies that any trajectory $\tau' \sim \pi'$ that reaches $G$ and passes through all bottleneck states in $B$ in $\delta(M^R_h)$ must also include $s$. Therefore, $\pi' \models_{\delta(M^R_h)} s$, which contradicts our initial assumption.

Thus, our assumption must be false, and the proposition holds: If $s$ is an implicit goal per human, then for the determinized human model of the robot $\delta(M^R_h)$, the state $s$ must be satisfied by every policy that satisfies the goal and its bottleneck states.
\end{proof}

\begin{proof}[Proof of Proposition 2]
Let $\mathbb{M}^R_h$ be a set of models defined over a finite state space $S$ and action space $A$, where $|S| = n$ and $|A| = m$. Note that $\mathbb{M}^R_h$ could potentially be infinite. We will show that the set of determinized models $\delta(\mathbb{M}^R_h)$ is finite.

Consider a single model $\mathcal{M}_i \in \mathbb{M}^R_h$. In its determinized version $\delta(\mathcal{M}_i)$, the state space remains the same: $|S'| = n$. For the action space in $\delta(\mathcal{M}_i)$, for each state-action pair $(s,a)$ in $\mathcal{M}_i$, we could have at most $n$ new actions in $\delta(\mathcal{M}_i)$, one for each possible next state. Thus, $|A'| \leq n \cdot m \cdot n = n^2m$.

To count the number of possible determinized models, we consider that for each state (n choices), for each possible action (at most $n^2m$ choices), we need to choose a resulting state (n choices). This gives us an upper bound of $n^{n^3m}$ possible determinized models.


Crucially, this upper bound is independent of the number of models in $\mathbb{M}^R_h$. Even if $\mathbb{M}^R_h$ is infinite, the number of unique determinized models is limited by the structure of the state and action spaces.

Therefore, we have:

$|\delta(\mathbb{M}^R_h)| \leq n^{n^3m}$

As $n$ and $m$ are finite, this upper bound is a finite number. Thus, $\delta(\mathbb{M}^R_h)$ is a finite set, even if $\mathbb{M}^R_h$ is infinite.

This finiteness arises from the determinization process itself: while the original models in $\mathbb{M}^R_h$ may have infinitely many different probability distributions over transitions, the determinization process collapses these probabilities to certainty, leading to a finite number of possible deterministic transition structures given the finite state and action spaces.
\end{proof}
